3D Morphable Face Models -- Past, Present and Future

In this paper, we provide a detailed survey of 3D Morphable Face Models over the 20 years since they were first proposed. The challenges in building and applying these models, namely capture, modeling, image formation, and image analysis, are still active research topics, and we review the state-of-the-art in each of these areas. We also look ahead, identifying unsolved challenges, proposing directions for future research and highlighting the broad range of current and future applications.

==> Ch-Open-Challenges.tex <==
%   ____                      _____ _           _ _                            
%  / __ \                    / ____| |         | | |                           
% | |  | |_ __   ___ _ __   | |    | |__   __ _| | | ___ _ __   __ _  ___  ___ 
% | |  | | '_ \ / _ \ '_ \  | |    | '_ \ / _` | | |/ _ \ '_ \ / _` |/ _ \/ __|
% | |__| | |_) |  __/ | | | | |____| | | | (_| | | |  __/ | | | (_| |  __/\__ \
%  \____/| .__/ \___|_| |_|  \_____|_| |_|\__,_|_|_|\___|_| |_|\__, |\___||___/
%        | |                                                    __/ |          
%        |_|                                                   |___/           
% http://patorjk.com/software/taag/#p=display&f=Big&t=Introduction

\section{Open Challenges}
\label{sec:challenges}

This chapter was moved to the specific chapters of the paper and global challenges where moved to the perspective chapter
